Revisiting the Effects of Leakage on Dependency Parsing

Recent work by S{\o}gaard (2020) showed that, treebank size aside, overlap between training and test graphs (termed leakage) explains more of the observed variation in dependency parsing performance than other explanations. In this work we revisit this claim, testing it on more models and languages. We find that it only holds for zero-shot cross-lingual settings. We then propose a more fine-grained measure of such leakage which, unlike the original measure, not only explains but also correlates with observed performance variation. Code and data are available here: https://github.com/miriamwanner/reu-nlp-project

==> stash.tex <==

\iffalse
\begin{table}[h]
    \centering
    \begin{tabular}{cc|cccc}
         \toprule
         System & Leakage & Regression & Explained & & \\
         System & Attributes & Score & Variance & MAE & Spearman's $\rho$ \\
        \midrule
        \multirow{3}{*}{Sogaard} & None & 0.1617 & 0.1430 & -7.2570 & -0.1942\\
        & Edges & 0.0914 & -0.1208 & -8.5922 & -0.1805\\
        & Nodes+Edges & 0.0846 & -0.1798 & -8.8302 & -0.1614\\
        \midrule
        \multirow{3}{*}{UDify (All)} & None & 0.2495 & 0.0466 & -13.0714 & -0.3601\\
        & Edges & 0.1465 & -0.0838 & -14.0123 & -0.0803\\
        & Nodes+Edges & 0.1344 & -0.1078 & -14.1556 & -0.0260\\
        %\midrule
        %\multirow{3}{*}{UDify (Zero-Shot)} & None & 0.3846 & 0.2629 & -17.5397 & -0.5812 \\
        %& Edges & 0.2207 & 0.1240 & -21.4603 & -0.4931 \\
        %& Nodes+Edges & 0.2210 & 0.1057 & -21.5065 & -0.5459 \\
        \bottomrule
    \end{tabular}
    \caption{Results calculated from entire UD data. All results reported over 5-fold cross validation. MAE: mean average error.}
    \label{tab:results}
\end{table}
\fi


\iffalse
\begin{table*}[]
    \centering
    \begin{tabular}{cc|cccc}
         \toprule
         System & Leakage Attributes & Regression Score & Explained Variance & $-$MAE & Spearman's $\rho$ \\
        \midrule
        \multirow{3}{*}{Sogaard} & None & 0.1466 & 0.0876 & -7.3671 & -0.1858\\
        & Edges & 0.0844 & -0.1384 & -8.6814 & -0.0227\\
        & Nodes+Edges & 0.0821 & -0.1652 & -8.8579 & -0.0314\\
        \midrule
        \multirow{3}{*}{UDpipe} & None & 0.2538 & -0.1483 & -7.4828 & -0.3199\\
        & Edges & 0.1511 & -0.0226 & -8.1176 & -0.1191\\
        & Nodes+Edges & 0.1443 & -0.0384 & -8.2315 & -0.0919\\
        \midrule
        \multirow{3}{*}{UDify (All)} & None & 0.2204 & 0.0102 & -13.2336 & -0.3544\\
        & Edges & 0.1421 & -0.0927 & -14.0232 & -0.0641\\
        & Nodes+Edges & 0.1341 & -0.1089 & -14.1007 & -0.0169\\
        \midrule
        \multirow{3}{*}{UDify (Zero-Shot)} & None & 0.2853 & 0.1438 & -19.0375 & -0.5544\\
        & Edges & 0.1982 & 0.1016 & -21.0340 & -0.4829\\
        & Nodes+Edges & 0.1746 & 0.0875 & -21.4302 & -0.3947\\
        \midrule
        \multirow{3}{*}{Stanza (All)} & None & \\
        & Edges & \\
        & Nodes+Edges & \\
        \bottomrule
    \end{tabular}
    \caption{Results calculated from modified UD data, which excludes all modifiers. All results reported over 5-fold cross validation. MAE: mean average error.}
    \label{tab:results}
\end{table*}
\fi


\iffalse
\begin{table*}[t]
    \centering
    \begin{tabular}{cc|cccc}
         \toprule
         System & Leakage Attributes & Regression Score & Explained Variance & $-$MAE & Spearman's $\rho$ \\
        \midrule
        \multirow{3}{*}{Sogaard} & None & 0.0537 & -0.1371 & -8.2482 & -0.2384\\
        & Edges & 0.0834 & -1.2021 & -9.4435 & 0.3904\\
        & Nodes+Edges & 0.0893 & -0.2103 & -8.1966 & 0.5384\\
        %\midrule
        %\multirow{3}{*}{UDpipe} & None & 0.1435 & -0.0714 & -8.2867 & -0.0382\\
        %& Edges & 0.1409 & -0.2628 & -9.2216 & 0.4137\\
        %& Nodes+Edges & 0.1668 & -0.2066 & -9.1931 & 0.5559\\
        \midrule
        \multirow{3}{*}{UDify (All)} & None & 0.1226 & -0.1707 & -14.6317 & -0.0815\\
        & Edges & 0.1742 & -0.3328 & -14.1815 & 0.5794\\
        & Nodes+Edges & 0.2174 & -0.1491 & -13.7151 & 0.6536\\
        %\midrule
        %\multirow{3}{*}{UDify (Zero-Shot)} & None & 0.0184 & -0.0230 & -24.0691 & 0.1913\\
        %& Edges & 0.2707 & 0.2095 & -18.2452 & 0.6092\\
        %& Nodes+Edges & 0.2459 & 0.2150 & -18.0380 & 0.5779\\
        %\midrule
        %\multirow{3}{*}{Stanza (All)} & None & \\
        %& Edges & \\
        %& Nodes+Edges & \\
        \bottomrule
    \end{tabular}
    \caption{Results calculated from modified UD data, which are three layer sub trees that consist of a node and its predecessor and successors. All results reported over 5-fold cross validation. MAE: mean average error.}
    \label{tab:newleakge}
\end{table*}
\fi

